Breaking the $3/4$ Barrier for Approximate Maximin Share

We study the fundamental problem of fairly allocating a set of indivisible goods among $n$ agents with additive valuations using the desirable fairness notion of maximin share (MMS). MMS is the most popular share-based notion, in which an agent finds an allocation fair to her if she receives goods worth at least her MMS value. An allocation is called MMS if all agents receive at least their MMS value. Since MMS allocations need not exist when $n>2$, a series of works showed the existence of approximate MMS allocations with the current best factor of $\frac34 + O(\frac{1}{n})$. However, a simple example in [DFL82, BEF21, AGST23] showed the limitations of existing approaches and proved that they cannot improve this factor to $3/4 + \Omega(1)$. In this paper, we bypass these barriers to show the existence of $(\frac{3}{4} + \frac{3}{3836})$-MMS allocations by developing new reduction rules and analysis techniques.

==> hard-instances.tex <==
\section{\boldmath Reduction to ordered normalized $(3/4+\delta)$-irreducible ($\delta$-ONI) instances}\label{hard-sec}
In this section, for any $\epsilon>0$ and $\delta \geq 4\epsilon/(1-4\epsilon)$ we show how to obtain a $\delta$-ONI instance $\I'$ from any arbitrary instance $\I$, such that from any $\alpha$-MMS allocation for $\I'$, one can obtain a $\min\left(3/4+\epsilon, (1-4\epsilon) \alpha \right)$-MMS allocation for $\I$. To obtain such an allocation, first we obtain a $(3/4+\epsilon)$-irreducible instance and we prove that the MMS value of no remaining agent drops by more than a multiplicative factor of $(1-4\epsilon)$. Then, we normalize and order the resulting instance which gives us a $\delta$-ONI instance (for $\delta \geq 4\epsilon/(1-4\epsilon)$). In the rest of this section, by $R_k$ we mean $R^{(3/4+\epsilon)}_k$ for $k \in [4]$.

We start with transforming the instance into an ordered one using $\mathtt{order}$ algorithm. Then we scale the valuations such that for all $i \in N$, $\mms_i = 1$. Then, as long as one of the reduction rules $R_1$, $R_2$, $R_3$ or $R_4$ is applicable, we apply $R_k$ for the smallest possible $k$. \cref{algo:reduce} shows the pseudocode of this procedure.

\begin{algorithm}[htb]
\caption{$\mathtt{reduce}((N, M, \mathcal{V}), \epsilon)$}
\label{algo:reduce}
\begin{algorithmic}[1]
\State $\I \leftarrow \mathtt{order}(N,M,\mathcal{V})$
\For{$i \in N$}
    \State $v_i \leftarrow v_i/\mms_i$
\EndFor
\While{$R^{(3/4+\epsilon)}_1$ is applicable}
    \State $\I \leftarrow R^{(3/4+\epsilon)}_1(\I)$
\EndWhile
\While{$R^{(3/4+\epsilon)}_2$ or $R^{(3/4+\epsilon)}_3$ or $R^{(3/4+\epsilon)}_4$ is applicable}
    \State $\I \leftarrow R^{(3/4+\epsilon)}_k(\I)$ for smallest possible $k$
\EndWhile
\State \Return $\I$.
\end{algorithmic}
\end{algorithm}
Since $R_1$ is a valid reduction rule for all the remaining agents $i$ by \cref{valid-rules}, $\mms_i \geq 1$ after applications of $R_1$. As an initial attempt, one might think that since $R_2$ and $R_3$ are also valid reductions, we can ignore them and only prove that after multiple applications of $R_4$, the MMS values remain to be at least $1-4\epsilon$. However, note that $R_2$ and $R_3$ are valid as long as the MMS values are $1$. Since $R_4$ could decrease the MMS values, once an $R_4$ is applied, we cannot assume $R_2$ and $R_3$ are valid.

Instead, in order to prove that the \mms~value of each agent $i$ remains at least $1 - 4\epsilon$, at each step after doing a reduction, we maintain a partition of the goods into $n$ bundles (where $n$ is the number of the remaining agents) and prove that the value of every bundle in this partition for $i$ is at least $1-4\epsilon$.


For a fixed agent $i$, let $P^1 = (P^1_1, P^1_2, \ldots, P^1_n)$ be an \mms~partition of $i$ right before applying any $R_k$ for $k>1$. We start with $P=P^1$ and after each reduction rule we alter $P$. After $R_2$ we do the following. By pigeonhole principle, there exists a bundle in $P$ with at least $3$ goods from $\{1, 2, \ldots, 2n+1\}$. Let $B$ be such a bundle and let $B_1$, $B_2$ and $B_3$ in $P$ be the bundles containing $2n-1$, $2n$ and $2n+1$ respectively. Note that these are not necessarily different bundles. Let $g_1, g_2, g_3 \in B \cap \{1,2,\ldots,2n+1\}$ and $g_1<g_2<g_3$. Replace $g_1$ with $2n-1$, $g_2$ with $2n$ and $g_3$ with $2n+1$. For all goods $g \in B \setminus\{g_1, g_2, g_3\}$, put $g$ in some arbitrary remaining bundle and \textbf{remove} $B$. Let $g_1 \in P^1_{j_1}$, $g_2 \in P^1_{j_2}$ and $g_3 \in P^1_{j_3}$. For all $k \in [3]$, we say bundle $P^1_{j_k}$ is ``touched'' by $R_2$.

The alternation of $P$ after $R_3$ is similar. By pigeonhole principle, there exists a bundle in $P$ with at least $4$ goods from $\{1, 2, \ldots, 3n+1\}$. Let $B$ be such a bundle and let $B_1$, $B_2$, $B_3$ and $B_4$ in $P$ be the bundles containing $3n-2$, $3n-1$, $3n$ and $3n+1$ respectively. Let $g_1, g_2, g_3, g_4 \in B \cap \{1,2,\ldots,2n+1\}$ and $g_1<g_2<g_3<g_4$. Replace $g_1$ with $3n-2$, $g_2$ with $3n-1$, $g_3$ with $3n$ and $g_4$ with $3n+1$. For all goods $g \in B \setminus\{g_1, g_2, g_3, g_4\}$, put $g$ in some arbitrary remaining bundle and \textbf{remove} $B$. Let $g_1 \in P^1_{j_1}$, $g_2 \in P^1_{j_2}$, $g_3 \in P^1_{j_3}$ and $g_4 \in P^1_{j_4}$. For all $k \in [4]$, we say bundle $P^1_{j_k}$ is ``touched'' by $R_3$.

The alteration of $P$ after $R_4$ is quite simple. If the goods $1$ and $2n+1$ belong to the same bundle $B$, we put all $g \in B \setminus \{1,2n+1\}$ in some arbitrary bundle and \textbf{remove} $B$. Otherwise, let $1 \in B_1$ and $2n+1 \in B_2$. We \textbf{merge} $B_1 \setminus \{1\}$ and $B_2 \setminus \{2n+1\}$. Let $1 \in P^1_{j_1}$ and $2n+1 \in P^1_{j_2}$. For all $k \in [2]$, we say $P^1_{j_k}$ is ``touched'' by $R_4$.

Note that the bundles in $P^1$ that are not touched by any reduction, remain to exist in $P$ and their value does not drop since they could only receive more goods or replace goods for more valuable goods. After each $R_2$ or $R_3$, one bundle is removed and after each $R_4$, either one bundle is removed or two bundles are merged. So each bundle in $P$ in the end of this procedure is either the result of merging some bundles or already exists in $P^1$.

\begin{observation}\label{removed}
    Let $P$ be the partition after an application of a reduction rule $R$ which removes a bag. For all bags $P_k$ in $P^1$, if $P_k$ is touched by $R$, then $P_k$ does not exists in $P$. 
\end{observation}
\begin{proof}
    Let $B$ be the bundle removed by $R$. All the bundles that are touched by $R$, have been merged into $B$ before applying $R$. Therefore, after applying $R$ and removing $B$, none of them exist.
\end{proof}
It only remains to prove that the bundles that are the result of merging touched bundles by $R_4$, have value at least $1-4\epsilon$.
\begin{lemma}\label{long-lemma}
    Let $B$ in $P$ be the result of merging touched bundles $P^1_1, \ldots, P^1_k$ in $P^1$ after a sequence of applied $R_4$s. Then $v_i(B) \geq 1 - 4\epsilon$.
\end{lemma}
\begin{proof}
    In each application of $R_4$, two goods $h$ and $\ell$ are removed. Let $h$ be the more valuable good. We call $h$ the heavy good and $\ell$ the light good of this application of $R_4$. By \cref{thm:vr-upper-bounds}, for all heavy goods $h$ and light goods $\ell$ we have, $v_i(h) < 3/4+\epsilon$ and $v_i(\ell) < 1/4+\epsilon/3$. 
    
    Note that $B$ is the result of applying $R_4$ for at most $k-1$ times. Let $H$ be the set of all heavy goods and $L$ be the set of all light goods that are removed during these reductions. Applications of other reduction rules which do not touch $B$ can only increase the value of $B$. Thus, without loss of generality, we can assume $B = (P_1 \cup P_2 \cup \ldots \cup P_n) \setminus (H \cup L)$ and we know $|H| = |L| \leq k-1$. Thus, it suffices to prove the following claim.
    \begin{claim}
        If $|(P_1 \cup P_2 \cup \ldots \cup P_k) \cap H| \leq k-1$ and $|(P_1 \cup P_2 \cup \ldots \cup P_k) \cap L| \leq k-1$, then $v_i(B) \geq v_i(P_1 \cup P_2 \cup \ldots \cup P_k) - v_i(H \cup L) \geq 1-4\epsilon$.
    \end{claim}
    The proof is by induction. For $k=2$, we have $v_i(P_1 \cup P_2) - v_i(H \cup L) \geq 2 - (\frac{3}{4}+\epsilon)-(\frac{1}{4}+\frac{\epsilon}{3}) > 1-4\epsilon$. 
    Now assume that the statement holds for all values of $k \leq k'-1$ and we prove it for $k = k'$. If there exists a bundle $B'$ such that $B' \cap H \neq \emptyset$ and $B' \cap L \neq \emptyset$, then at most $k-2$ heavy goods and at most $k-2$ light goods are removed from the other bundles and by induction hypothesis, $v_i(B) \geq 1-4\epsilon$ \todo{...}. So we can assume that for all $j \in [k]$, $P_j \cap H = \emptyset$ or $P_j \cap L = \emptyset$. Let $S_1 := \{j \in [k] \mid P_j \cap H = \emptyset\}$ and $S_2 := \{j \in [k] \mid P_j \cap L = \emptyset\}$. If there exist bundles $B'$ and $B''$ such that $|B' \cap H| \geq 2$ and $|B'' \cap L| \geq 2$, induction hypothesis holds after removing $B'$ and $B''$. Therefore, for all $j \in S_1$, $|P_j \cap L|=1$ or for all $j \in S_2$, $|P_j \cap H|=1$. Hence, there are at least $k-1$ bundles $P_1, \ldots, P_{k-1}$ such that $|P_j \cap (H \cup L)| = 1$ for $j \in [k-1]$. We have
    \begin{align*}
        v_i(B) \geq \sum_{j \in [k-1]} v_i\left(P_j \setminus (H \cup L)\right) &= \sum_{j \in [k-1]} \left(v_i(P_j) - v_i(P_j \cap (H \cup L))\right) \\
        &> (k-1)\left(1 - (\frac{3}{4}+\epsilon)\right) &\tag{$v_i(P_j \cap (H \cup L)) \leq \frac{3}{4}+\epsilon$}\\
        &= (k-1)(\frac{1}{4}-\epsilon) \geq 1-4\epsilon. &\tag{for $k>4$}
    \end{align*}
    It remains to prove the lemma when $k=3$ and $k=4$. If there are two bundles $P_1$ and $P_2$ such that $|P_1 \cap L| = |P_2 \cap L| = 1$, $v_i(B) \geq v_i(P_1 \setminus L) + v_i(P_2 \setminus L) > 2\left(1 - (\frac{1}{4}+\frac{\epsilon}{3})\right) > 1-4\epsilon$. Otherwise, for $k=3$, there are two bundles $P_1$ and $P_2$ such that $|P_1 \cap H|=|P_2 \cap H|=1$ and $|P_3 \cap L|=2$. Then, 
    \begin{align*}
        v_i(B) &= v_i(P_1 \setminus H) + v_i(P_2 \setminus H) + v_i(P_3 \setminus L) \\
        &> 2\left(1 - (\frac{3}{4}+\epsilon)\right) + \left(1 - 2(\frac{1}{4}+\frac{\epsilon}{3})\right) \\
        &= 1 - \frac{8\epsilon}{3} > 1-4\epsilon.
    \end{align*}
    For $k=4$, we have $|P_1 \cap H|=|P_2 \cap H|=|P_3 \cap H|=1$ and $|P_4 \cap L|=3$. Then, 
    \begin{align*}
        v_i(B) &= v_i(P_1 \setminus H) + v_i(P_2 \setminus H) + v_i(P_3 \setminus H) + v_i(P_4 \setminus L) \\
        &> 3\left(1 - (\frac{3}{4}+\epsilon)\right) + \left(1 - 3(\frac{1}{4}+\frac{\epsilon}{3})\right) = 1-4\epsilon.
\qedhere    \end{align*}
\end{proof}
\begin{lemma}\label{missing-factor}
    Given an instance $\I = (N, M, \mathcal{V})$ and $\epsilon \geq 0$, let $\I' = (N', M', \mathcal{V}') = \mathtt{reduce}(\I, \epsilon)$. For all agents $i \in N'$, $\mms_i(\I') \geq 1-4\epsilon$.
\end{lemma}
\begin{proof}
    By \cref{removed}, for all remaining bundles $P_j$ in $P$ in the end of \cref{algo:new}, $P_j$ is either untouched or is the result of merging some touched bundles. The untouched bundles in $P$ also exist in $P^1$ and their value does not drop since they could only receive more goods or replace goods for more valuable goods. Therefore, if $P_j$ is untouched, $v_i(P_j) \geq v_i(P^1_j) = 1 > 1-4\epsilon$. Otherwise, by \cref{long-lemma}, $v_i(P_j) \geq 1-4\epsilon$.
\end{proof}
\begin{theorem}
    Given an instance $\I$ and $\epsilon \geq 0$, let $\hat{\I} = \mathtt{order}(\mathtt{normalize}(\mathtt{reduce}(\I, \epsilon)))$. Then $\hat{\I}$ is ordered, normalized and $(\frac{3}{4}+\frac{4\epsilon}{1-4\epsilon})$-irreducible ($\frac{4\epsilon}{1-4\epsilon}$-ONI). Furthermore, from any $\alpha$-MMS allocation of $\hat{\I}$ one can obtain a $\min(3/4+\epsilon, (1-4\epsilon)\alpha)$-MMS allocation of $\I$.  
\end{theorem}
\begin{proof}
    In $\mathtt{reduce}$, as long as $R^{(3/4+\epsilon)}_1$ is applicable, we apply it. Once it is not applicable anymore, for all remaining agents $i$, $v_i(1)<3/4+\epsilon$. In the rest of the procedure $\mathtt{reduce}$, we do not increase the value of any good for any agent. Therefore, $R^{(3/4+\epsilon)}_1$ remains inapplicable. As long as one of the rules $R^{(3/4+\epsilon)}_k$ is applicable for $k \in \{2,3,4\}$, we apply it. Therefore, $\mathtt{reduce}(\I, \epsilon)$ is $(3/4+\epsilon)$-irreducible. Let $\I' = (N',M',\mathcal{V}') = \mathtt{reduce}(\I, \epsilon)$. Since $\mms_i(\I') \geq 1-4\epsilon$ (by \cref{missing-factor}), $\mathtt{normalize}$ can increase the value of each good by a multiplicative factor of at most $1/(1-4\epsilon)$. Therefore, after ordering the instance, none of the rules $R^\beta_k$ for $k \in [4]$ would be applicable for $\beta \geq \frac{3/4+\epsilon}{1-4\epsilon} = \frac{3}{4}+\frac{4\epsilon}{1-4\epsilon}$. Hence, $\mathtt{order}(\mathtt{normalize}(\mathtt{reduce}(\I, \epsilon)))$ is $\beta$-irreducible for $\beta \geq \frac{3}{4}+\frac{4\epsilon}{1-4\epsilon}$ and it is of course ordered. Since $\mathtt{order}$ does not change the multiset of the values of the goods each agents, the instance remains normalized.

    Now let us assume $A$ is an $\alpha$-MMS allocation for $\hat{\I} = \mathtt{order}(\mathtt{normalize}(\mathtt{reduce}(\I, \epsilon)))$. By \cref{order-preserves}, we can obtain an allocation $B$ which is $\alpha$-MMS for $\mathtt{normalize}(\mathtt{reduce}(\I, \epsilon))$. \cref{thm:normalize} implies that $B$ is $\alpha$-MMS for $\I' = (N', M', \mathcal{V}') = \mathtt{reduce}(\I, \epsilon)$. For all agents $i \in N \setminus N'$, $v'_i(B_i) = v_i(B_i)/\mms_i(\I)$. Therefore, 
    \begin{align*}
        v_i(B_i) &= v'_i(B_i)\mms_i(\I) \\
        &\geq \alpha\mms_i(\I')\mms_i(\I) \tag{$B$ is $\alpha$-MMS for $\I'$}\\
        &\geq \alpha(1-4\epsilon)\mms^n_{v_i}(M). \tag{$\mms^n_{v'_i}(M) \geq 1-4\epsilon$ by \cref{missing-factor}}
    \end{align*}
    Thus, $B$ gives all the agents in $N'$, $\alpha(1-4\epsilon)$ fraction of their MMS. All agents in $N \setminus N'$ receive $(3/4+\epsilon)$ fraction of their MMS value. Therefore, the final allocation is a $\min(3/4+\epsilon, (1-4\epsilon)\alpha)$-MMS allocation of $\I$.  
\end{proof}
